Neural mixture model association of seismic phases

Seismic phase association is the task of grouping phase arrival picks across a seismic network into subsets with common origins. Building on recent successes in this area with machine learning tools, we introduce a neural mixture model association algorithm (Neuma), which incorporates physics-informed neural networks and mixture models to address this challenging problem. Our formulation assumes explicitly that a dataset contains real phase picks from earthquakes and noise picks resulting from phase picking mistakes and fake picks. The problem statement is then to assign each observation to either an earthquake or noise. We iteratively update a set of hypocenters and magnitudes while determining the optimal class assignment for each pick. We show that by using a physics-informed Eikonal solver as the forward model, we can impose stringent quality control on surviving picks while maintaining high recall. We evaluate the performance of Neuma against several baseline algorithms on a series of challenging synthetic datasets and the 2019 Ridgecrest, California sequence. Neuma outperforms the baselines in precision and recall for each of the synthetic datasets. Furthermore, it detects an additional 3285 more earthquakes than the best baseline on the Ridgecrest dataset (13.5%), while substantially improving the hypocenters.

==> Sections/Acknowledgements.tex <==
% \section*{Acknowledgements}


==> old_files/4-Method.tex <==


\section{Method}\label{Sec:SV}

\subsection{E-step}

\begin{equation}
    Q(\theta | x, z, G) = \mathbb{E}_{z,G|x} \left[\, \log p(x, z, G \, | \, \theta)\right] \\
\end{equation}

\begin{equation}
    Q(\theta | x, z, G) = \sum_{i=1}^N \mathbb{E}_{G|x} \left[I(G_i)\right] \left(\log w + \log (1-w) + \log{\U(x_i)} + \\
    \sum_{k=1}^K \mathbb{E}_{z|x}\left[I(z_i=k)\right] \left(\log \varphi_k + \log p(x_i | \theta_k) \right)\right)
\end{equation}

\begin{equation}
    \mathbb{E}_{G|x} \left[I(G_i)\right] = p(G_i | x_i) = \frac{p(x_i | G_i) p(G_i)}{p(x_i)} = \frac{w \sum_{k=1}^K \varphi_k p(x_i | \theta_k)}{w \sum_{k=1}^K \varphi_k p(x_i | \theta_k) + (1-w)\U(x_i)}  = \nu_i \\
\end{equation}
\begin{equation}
    \mathbb{E}_{z|x}\left[I(z_i=k)\right] = p(z_i=k | x_i) = \frac{\varphi_k p(x_i | \theta_k)}{\sum_{j=1}^K \varphi_j p(x_i | \theta_j)} = \gamma_{ik}
\end{equation}


Then the expectation of the log likelihood becomes,
\begin{equation}
    Q(\theta | x, z, G) = \sum_{i=1}^N \nu_i \left(\log w + \log (1-w) + \log{\U(x_i)} + \\
    \sum_{k=1}^K \gamma_{ik} \left(\log \varphi_k + \log p(x_i | \theta_k) \right)\right)
\end{equation}

\subsection{M-step}
\begin{equation}
 \hat{\theta} = \text{argmax}_\theta \, Q(\theta | x, z, G)
\end{equation}



\paragraph{The E-step}

The likelihood function is the following,
\begin{equation}
    p(x) =  \prod_i^N p(x_i)
\end{equation}
where for each $p(x_i)$ we have,

% \begin{align}
%     p(x_i) = \sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1} p_\U(x_i), ~~~\sum_k^{K+1}\phi_k = 1
% \end{align}

\begin{align}
    p(x_i) = (1-w_i)\sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+w_i p_\U(x_i), ~~~\sum_k^{K}\phi_k = 1
\end{align}

\begin{align}
    p(x_i) = (1-w_i)\sum_k^K\phi_kp_\N(x^t_i,\mu_k,\Lambda_k)p_A(x^a_i,\mu_k,\Lambda_k)+w_i p_\U(x^t_i)p_A^G(x^a_i), ~~~\sum_k^{K}\phi_k = 1
\end{align}


Eq 4 in Weiqiang's stay the same. 

\begin{align}
    \gamma_{i,k} = \frac{\phi_kp_\N(x_i,\mu_k,\Lambda_k)}{\sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1} p_\U(x_i)}
\end{align}
\begin{align}
    \gamma_{i,k} = \frac{\phi_kp_\N(x^t_i,\mu_k,\Lambda_k)p_A(x^a_i,\mu_k,\Lambda_k)}{\sum_k^K\phi_kp_\N(x^t_i,\mu_k,\Lambda_k)p_A(x^a_i,\mu_k,\Lambda_k)+\phi_{K+1} p_\U(x^t_i)p_A^G(x^a_i)}
\end{align}
for all $k\in[K]$, and 

\begin{align}
    \gamma_{i,K+1} = \frac{\phi_{K+1} p_\U(x_i)}{\sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1} p_\U(x_i)}
\end{align}
\begin{align}
    \gamma_{i,K+1} = \frac{\phi_{K+1} p_\U(x^t_i)p_A^G(x^a_i)}{\sum_k^K\phi_kp_\N(x^t_i,\mu_k,\Lambda_k)p_A(x^a_i,\mu_k,\Lambda_k)+\phi_{K+1} p_\U(x^t_i)p_A^G(x^a_i)}
\end{align}
Then eq 6 and 7 in Weiqiang's paper stay the same. 


% In the case we use Zach's idea, we have

% \begin{align*}
%     p(x_i) = \sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1}, ~~~\sum_k^{K+1}\phi_k = 1
% \end{align*}

% Eq 4 in Weiqiang's stay the same. 

% \begin{align*}
%     \gamma_{i,k} = \frac{\phi_kp_\N(x_i,\mu_k,\Lambda_k)}{\sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1}}
% \end{align*}
% for all $k\in[K]$, and 

% \begin{align*}
%     \gamma_{i,K+1} = \frac{\phi_{K+1}}{\sum_k^K\phi_kp_\N(x_i,\mu_k,\Lambda_k)+\phi_{K+1}}
% \end{align*}
% Then eq 6 and 7 in Weiqiang's paper stay the same. 


\subsection{Implementation}
Our implementation of the E-M equations includes a few changes from that described by \citet{zhu_earthquake_2022}. We found that if the uncertainties on the likelihood functions, i.e. $p_\N(x_i,\mu_k,\Lambda_k)$ and $p_A(x^a_i,\mu_k,\Lambda_k)$, were set to values representative of the true velocity model and picking errors right from the start, that the E-M would converge to a poor minimum by assigning most picks automatically to the garbage class. The reason for this is because if the initial hypocenters assigned to the $K$ clusters are not sufficiently close to the true position, that the E-step assignments for $\gamma$ would always start out being effectively zero for all picks, which is lower than the probability of the garbage distribution. To circumvent this problem, we designed an implementation that instead has a warmup period in which the garbage variables are turned off (i.e. $\gamma_{i,K+1}=0$) to allow for the $K$ hypocenters to first be optimized. During this period, we also decay the numerical values of $\Lambda_k$ for both the travel times and the amplitudes. At iteration 1, $\Lambda_k$ is set to 5 times the actual (assumed) uncertainty of the travel times and amplitudes, and then is decayed linearly to the actual uncertainty over 10 warmup iterations. The initial value of the uncertainty was chosen as a compromise being much larger than the true (final) uncertainty, but not so large that all clusters have the same likelihood of pick assignment. After the warmup period is over, $\gamma_{i,K+1}$ is computed at each iteration rather than being forced to zero, and $\Lambda_k$ is set to the constant values taken at the final iteration of the warmup. We found that the E-M converged typically within about 5 iterations after the warmup period was finished.

The forward model used to compute $\mu_k$ for Neuma is an EikoNet \citep{smith_eikonet_2020}, a physics-informed deep neural network trained to solve the Eikonal equation for ray tracing. We use a simplified network architecture to maximize computational efficiency, with 5 dense layers of 128 neurons followed by exponential linear unit activations. We perform the M-step update of the $K$ hypocenters using the Adam optimizer \citep{kingma_adam:_2014} in a non-stochastic (all data points used) fashion.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/garbage_amp_dist.pdf}
    \caption{Garbage pick amplitude distribution.}
    \label{fig:garbageampdist}
\end{figure}
%% statistics from GaMMA picks
%% mean of log10(PGV) = -5.46
%% std of log10(PGV) = -0.72
%% TODO: add statistics from Neuma picks
